Stochastic Optimization with Parametric Cost Function Approximations

A widely used heuristic for solving stochastic optimization problems is to use a deterministic rolling horizon procedure, which has been modified to handle uncertainty (e.g. buffer stocks, schedule slack). This approach has been criticized for its use of a deterministic approximation of a stochastic problem, which is the major motivation for stochastic programming. We recast this debate by identifying both deterministic and stochastic approaches as policies for solving a stochastic base model, which may be a simulator or the real world. Stochastic lookahead models (stochastic programming) require a range of approximations to keep the problem tractable. By contrast, so-called deterministic models are actually parametrically modified cost function approximations which use parametric adjustments to the objective function and/or the constraints. These parameters are then optimized in a stochastic base model which does not require making any of the types of simplifications required by stochastic programming. We formalize this strategy and describe a gradient-based stochastic search strategy to optimize the parameters.

==> images/ChargeRates_All/forecast_performance.tex <==
\begin{tabular}{|l|c|c|c|c|}
\hline
&\textbf{$\gamma =0.25$}&\textbf{$\gamma =0.5$}&\textbf{$\gamma =0.75$}&\textbf{$\gamma =1$}\\\hline
\textbf{Constant}&0.10&0.10&0.09&0.09\\\hline
\textbf{Lookup}&0.17&0.15&0.15&0.16\\\hline
\textbf{Expo}&0.11&0.16&0.16&0.14\\\hline
\textbf{Capacity Con.}&0.00&0.00&0.00&0.00\\\hline
\end{tabular}


==> images/ChargeRates_All/theta_CC.tex <==
\begin{tabular}{|l|c|c|c|}
\hline
&\textbf{Improvement}&\textbf{$\theta_{1}$}&\textbf{$\theta_{2}$}\\\hline
\textbf{$\gamma = $0.05}&0.0000&0.9998&0.0000\\\hline
\textbf{$\gamma = $0.15}&0.0002&0.9912&0.0000\\\hline
\textbf{$\gamma = $0.25}&0.0000&1.0000&0.0000\\\hline
\textbf{$\gamma = $0.5}&-0.0001&0.9895&0.0000\\\hline
\textbf{$\gamma = $1}&0.0018&0.9403&0.0000\\\hline
\end{tabular}


==> images/ChargeRates_All/theta_exp.tex <==
\begin{tabular}{|l|c|c|c|}
\hline
&\textbf{Improvement}&\textbf{$\theta_{1}$}&\textbf{$\theta_{2}$}\\\hline
\textbf{$\gamma = $0.05}&0.1342&0.4677&-0.0623\\\hline
\textbf{$\gamma = $0.15}&0.2217&0.5688&-0.0684\\\hline
\textbf{$\gamma = $0.25}&0.1936&1.1904&-0.1249\\\hline
\textbf{$\gamma = $0.5}&0.1100&1.0556&-0.0679\\\hline
\textbf{$\gamma = $1}&0.0934&1.2519&-0.0852\\\hline
\end{tabular}


==> images/ChargeRates_All/theta_lookup.tex <==
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|}
\hline
&\textbf{Improvement}&\textbf{$\theta_{1}$}&\textbf{$\theta_{2}$}&\textbf{$\theta_{3}$}&\textbf{$\theta_{4}$}&\textbf{$\theta_{5}$}&\textbf{$\theta_{6}$}&\textbf{$\theta_{7}$}&\textbf{$\theta_{8}$}\\\hline
\textbf{$\gamma = $0.05}&0.1054&0.8670&0.7982&0.8017&0.7836&0.7201&0.6223&0.5033&0.4817\\\hline
\textbf{$\gamma = $0.15}&0.1898&0.5034&0.3505&0.8940&1.0116&0.3722&0.4409&0.2704&0.3884\\\hline
\textbf{$\gamma = $0.25}&0.0783&0.6356&1.2542&0.9850&0.9813&0.9406&0.6091&0.2439&0.1694\\\hline
\textbf{$\gamma = $0.5}&0.1112&0.1548&0.1694&0.3594&0.5356&0.7720&0.8557&0.8351&0.8291\\\hline
\textbf{$\gamma = $1}&0.0662&1.0334&1.0488&0.7105&0.6985&0.5581&1.1686&0.9312&1.0418\\\hline
\end{tabular}


==> images/ChargeRates_All/theta_single.tex <==
\begin{tabular}{|l|c|c|}
\hline
&\textbf{Improvement}&\textbf{$\theta_{1}$}\\\hline
\textbf{$\gamma = $0.05}&0.1041&0.1571\\\hline
\textbf{$\gamma = $0.15}&0.0431&0.8656\\\hline
\textbf{$\gamma = $0.25}&0.0512&0.8263\\\hline
\textbf{$\gamma = $0.5}&0.1742&0.0617\\\hline
\textbf{$\gamma = $1}&0.3230&0.2571\\\hline
\end{tabular}


==> images/ForecastQuality_All/theta_CC.tex <==
\begin{tabular}{|l|c|c|c|}
\hline
&\textbf{Improvement}&\textbf{$\theta_{1}$}&\textbf{$\theta_{2}$}\\\hline
\textbf{$\sigma_f = $20}&0.0000&0.9665&0.0000\\\hline
\textbf{$\sigma_f = $30}&0.0000&0.9664&0.0000\\\hline
\textbf{$\sigma_f = $40}&0.0000&0.9669&0.0000\\\hline
\textbf{$\sigma_f = $50}&-0.0573&0.9668&0.0007\\\hline
\end{tabular}


==> images/ForecastQuality_All/theta_exp.tex <==
\begin{tabular}{|l|c|c|c|}
\hline
&\textbf{Improvement}&\textbf{$\theta_{1}$}&\textbf{$\theta_{2}$}\\\hline
\textbf{$\sigma_f = $20}&0.0472&0.2548&-0.0262\\\hline
\textbf{$\sigma_f = $30}&0.1450&0.1594&-0.0291\\\hline
\textbf{$\sigma_f = $40}&0.1411&0.3075&-0.0377\\\hline
\textbf{$\sigma_f = $50}&0.1608&0.1550&-0.0371\\\hline
\end{tabular}


==> images/ForecastQuality_All/theta_lookup.tex <==
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|}
\hline
&\textbf{Improvement}&\textbf{$\theta_{1}$}&\textbf{$\theta_{2}$}&\textbf{$\theta_{3}$}&\textbf{$\theta_{4}$}&\textbf{$\theta_{5}$}&\textbf{$\theta_{6}$}&\textbf{$\theta_{7}$}&\textbf{$\theta_{8}$}\\\hline
\textbf{$\sigma_f = $20}&0.0903&0.6718&0.4310&0.1368&0.1404&0.1136&0.0902&0.0330&0.0312\\\hline
\textbf{$\sigma_f = $30}&0.1634&0.6496&0.4301&0.0713&0.0137&0.0037&0.0127&0.0005&0.0291\\\hline
\textbf{$\sigma_f = $40}&0.1802&0.5435&0.1163&0.0757&0.0073&0.0040&0.0040&0.0040&0.0409\\\hline
\textbf{$\sigma_f = $50}&0.1751&0.6127&0.3935&0.2243&0.4018&0.3879&0.4642&0.4663&0.4234\\\hline
\end{tabular}


==> images/ForecastQuality_All/theta_single.tex <==
\begin{tabular}{|l|c|c|}
\hline
&\textbf{Improvement}&\textbf{$\theta_{1}$}\\\hline
\textbf{$\sigma_f = $20}&0.0570&0.4331\\\hline
\textbf{$\sigma_f = $30}&0.1256&0.1660\\\hline
\textbf{$\sigma_f = $40}&0.1332&0.2290\\\hline
\textbf{$\sigma_f = $50}&0.1646&0.1251\\\hline
\end{tabular}

